Optimization of Quantum Systems Emulation via a Variant of the Bandwidth Minimization Problem

This paper introduces weighted-BMP, a variant of the Bandwidth Minimization Problem (BMP), with a significant application in optimizing quantum emulation. Weighted-BMP optimizes particles ordering to reduce the emulation costs, by designing a particle interaction matrix where strong interactions are placed as close as possible to the diagonal. We formulate the problem using a Mixed Integer Linear Program (MILP) and solve it to optimality with a state of the art solver. To strengthen our MILP model, we introduce symmetry-breaking inequalities and establish a lower bound. Through extensive numerical analysis, we examine the impacts of these enhancements on the solver's performance. The introduced reinforcements result in an average CPU time reduction of 25.61 percent. Additionally, we conduct quantum emulations of realistic instances. Our numerical tests show that the weighted-BMP approach outperforms the Reverse Cuthill-McKee (RCM) algorithm, an efficient heuristic used for site ordering tasks in quantum emulation, achieving an average memory storage reduction of 24.48 percent. From an application standpoint, this study is the first to apply an exact optimization method, weighted-BMP, that considers interactions for site ordering in quantum emulation pre-processing, and shows its crucial role in cost reduction. From an algorithmic perspective, it contributes by introducing important reinforcements and lays the groundwork for future research on further enhancements, particularly on strengthening the weak linear relaxation of the MILP.

==> conclusion.tex <==



This paper presented a realistic implementation of a Large-scale Deterministic Network (LDNs) to provide deterministic E2E latency and bounded jitter in large-scale IP networks. At the data plane, high scalability is achieved considering an asynchronous cyclic scheduling with 3 queues and a low complexity forwarding in $O(1)$. 
To ensure deterministic performance, the traffic is shaped at I-GWs using gate-control queues that allow achieving a granularity of 1.5 kB, improving traditional methods. Detailed analysis shows that LDN can guarantee a bounded E2E queuing delay of $(2h-1)T$ for a $h$-hop flow and a $2T$ jitter bound. 
We also presented CGRR, a control plane algorithm for admission control, to maximize the accepted traffic by computing the best feasible shaping parameters and paths for a batch of incoming flows. 
Besides, we also verified the performance of LDN through a PoC implementation and simulations. We showed that the proposed CGRR algorithm outperforms traditional OSPF routing by up to 40\% in terms of traffic acceptance. 
Our results confirm that LDN is suitable to large-scale IP networks. 







==> problem_statement.tex <==


